TumorChain: Interleaved Multimodal Chain-of-Thought Reasoning for Traceable Clinical Tumor Analysis

Accurate tumor analysis is central to clinical radiology and precision oncology, where early detection, reliable lesion characterization, and pathology-level risk assessment guide diagnosis and treatment planning. Chain-of-Thought (CoT) reasoning is particularly important in this setting because it enables step-by-step interpretation from imaging findings to clinical impressions and pathology conclusions, improving traceability and reducing diagnostic errors. Here, we target the clinical tumor analysis task and build a large-scale benchmark that operationalizes a multimodal reasoning pipeline, spanning findings, impressions, and pathology predictions. We curate TumorCoT, a large-scale dataset of 1.5M CoT-labeled VQA instructions paired with 3D CT scans, with step-aligned rationales and cross-modal alignments along the trajectory from findings to impression to pathology, enabling evaluation of both answer accuracy and reasoning consistency. We further propose TumorChain, a multimodal interleaved reasoning framework that tightly couples 3D imaging encoders, clinical text understanding, and organ-level vision-language alignment. Through cross-modal alignment and iterative interleaved causal reasoning, TumorChain grounds visual evidence, aggregates conclusions, and issues pathology predictions after multiple rounds of self-refinement, improving traceability and reducing hallucination risk. Experiments show consistent improvements over strong baselines in lesion detection, impression generation, and pathology classification, and demonstrate strong generalization on the DeepTumorVQA benchmark. These results highlight the potential of multimodal reasoning for reliable and interpretable tumor analysis in clinical practice. Detailed information about our project can be found on our project homepage at https://github.com/ZJU4HealthCare/TumorChain.

==> table/cot_eval.tex <==
\begin{table}[t]
\caption{CoT-Eval comparison of TumorChain with other \textbf{Reasoning VLMs} on \texttt{TumorCoT}.}
\label{tab:cot_eval}
\begin{center}
 \renewcommand\tabcolsep{24pt}
 \renewcommand{\arraystretch}{1}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
\multirow{2}{*}{\textbf{Reasoning Models}}
& \multicolumn{4}{c}{\textbf{CoT-Eval}} \\
\cmidrule(rl){2-5}
 & $S_{FC}$ & $S_{IC}$ & $S_{LRC}$ & $CoT_{e}$ \\
\midrule
Claude3-Haiku     & 59.31 & 43.66 & 30.80 & 43.21  \\
Gemini2.0-Flash    & 63.10 & 57.69 & 45.12 & 54.28  \\
GPT-5-Mini         & \textbf{64.22} & \textbf{66.42} & \textbf{55.09} & \textbf{61.23}  \\
\midrule
Qwen2.5-VL-7B      & 49.15 & 22.89 & 12.09 & 26.45 \\
InternVL-2.5-8B    & 56.66 & 57.92 & 47.05 & 53.19  \\
MiniCPM-V-4.5-9B   & 60.51 & 58.52 & 45.44 & 53.89 \\
\midrule
HealthGPT-3.8B     & 49.64 & 49.68 & 37.15 & 44.65 \\
Lingshu-7B         & 52.51 & 31.93 & 16.46 & 31.92 \\
MedVLM-R1-2B       & 40.25 & 36.05 & 21.23 & 31.38 \\
\midrule
\textbf{TumorChain-3B} & 62.37 & 49.99 & 35.68 & 47.98 \\
\textbf{TumorChain-7B} & 61.75 & 62.60 & 52.57 & 58.33 \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}



==> table/deeptumorVQA.tex <==
\begin{table}[t]
\caption{Comparison of TumorChain with other VLMs on the public DeepTumorVQA benchmark.}
\label{tab:deeptumorVQA}
\begin{center}
 \renewcommand\tabcolsep{18pt}
  \renewcommand{\arraystretch}{1.1}
 \resizebox{\linewidth}{!}{
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Measurement} & \textbf{Recognition} & \textbf{Visual Reasoning} & \textbf{Medical Reasoning} \\
\midrule
\rowcolor{gray!5}
\multicolumn{5}{c}{\textit{Commercial Models}} \\
\midrule
Claude3-Haiku         & 28.70 & 38.70  & 31.53  & 34.81  \\
Gemini2.0-Flash       & 23.63  & 50.88 & 33.81  & 35.06 \\
GPT-5-mini             & 40.42  & 49.29  & 35.57  & 29.87 \\
\midrule
\rowcolor{gray!5}
\multicolumn{5}{c}{\textit{Generalist Models}} \\
\midrule
Qwen2.5-VL-7B     & 27.44 & 45.31 & 36.94 & 37.04  \\
InternVL-2.5-8B   & 25.14 & 50.06 & 31.35 & 44.20 \\
MiniCPM-V4.5-9B   & 34.13 & 50.14 & 33.69 & 42.86 \\
\midrule
\rowcolor{gray!5}
\multicolumn{5}{c}{\textit{2D Medical Models}} \\
\midrule
HealthGPT-3.8B      & 21.12 & 43.32 & 30.68 & 39.75 \\
Lingshu-7B          & 30.83 & 50.24 & 36.19 & 37.78 \\
MedVLM-R1-2B        & 26.54 & \textbf{56.41} & \underline{38.27} & 33.33 \\
\midrule
\rowcolor{gray!5}
\multicolumn{5}{c}{\textit{3D Medical Models}} \\
\midrule
RadFM          & 24.03  & 50.19  & \textbf{39.82}  & 30.87  \\
M3D-Phi3-4B    & 24.60  & 29.53  & 23.22  & 23.70 \\
\rowcolor{blue!5}
\textbf{TumorChain-7B (Zero-shot)}      & 24.78  & \underline{53.62} & 36.97 & \textbf{45.93} \\
\rowcolor{blue!5}
\textbf{TumorChain-7B+DeepTumorVQA}     &   &   &   &   \\
\rowcolor{blue!5}
\textbf{TumorChain-7B+DeepTumorVQACoT}  &   &   &   &   \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}


==> table/module_ablation.tex <==
\begin{table*}[t]
\centering
\caption{Ablation study of the effect of individual modules in TumorChain. Organ Pos. = Organ Position, Tumor Pos. = Tumor Position, Seg. Loc. = Segmentation Localization. }
\label{tab:module_ablation}
  \renewcommand{\arraystretch}{1}
\resizebox{\textwidth}{!}{
\begin{tabular}{ccccccccccccccc}
\toprule
\multicolumn{2}{c}{\textbf{Modules}} 
& \multicolumn{2}{c}{\textbf{Position}} 
& \multicolumn{6}{c}{\textbf{Lesion Attributes}} 
& \multicolumn{3}{c}{\textbf{TNM Prediction}} 
& \multirow{3}{*}{\textbf{\begin{tabular}{@{}c@{}}CoT-\\Report\end{tabular} }} 
& \multirow{3}{*}{\textbf{Avg.}} \\
\cmidrule(rl){1-2} \cmidrule(rl){3-4} \cmidrule(rl){5-10} \cmidrule(rl){11-13}
\textbf{CoT} & \textbf{IIR} & \begin{tabular}{@{}c@{}}Organ\\Pos.\end{tabular} & \begin{tabular}{@{}c@{}}Tumor\\Pos.\end{tabular} & \begin{tabular}{@{}c@{}}Seg.\\Loc.\end{tabular} & Shape & Boundary & Density & Count & Others & Tumor & Node & Met.  \\
\midrule
- & - & 99.92 & 97.45 & 78.95 & 75.78 & 74.60 & 80.18 & 82.82 & 78.75 & 84.37 & 59.29 & 66.85 & 79.83 & 79.90 \\
- & \faCheckCircle & 99.91 & 97.10 & 82.75 & 78.43 & 82.57 & 82.79 & 84.26 & 84.16 & 88.34 & 60.76 & 68.12 & 80.26 & 82.45 \\
\faCheckCircle & - & 99.87 & 97.55 & 79.36 & 79.52 & 74.62 & 81.46 & 80.60 & 79.20 & 84.65 & 60.32 & 65.87 & 81.06 & 80.34 \\
\rowcolor{blue!5} \faCheckCircle & \faCheckCircle & 99.97 & 97.57 & 86.88 & 82.28 & 84.52 & 85.05 & 86.20 & 86.57 & 88.83 & 61.63 & 71.07 & 82.36 & 84.41 \\
\bottomrule
% \vspace{-8mm}
\end{tabular}}
\end{table*}


==> table/orin_cot_eval.tex <==

\begin{table}[t]
\caption{CoT-Eval comparison of TumorChain with other \textbf{Reasoning VLMs} on \texttt{TumorCoT}.}
\label{tab:orin_cot_eval}
\begin{center}
 \renewcommand\tabcolsep{10pt}
  \renewcommand{\arraystretch}{1.1}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
\multirow{2}{*}{\textbf{Reasoning Models}} 
& \multicolumn{4}{c}{\textbf{CoT-Eval}} 
&  \multirow{2}{*}{\textbf{Liver}} &  \multirow{2}{*}{\textbf{Pancreas}} &  \multirow{2}{*}{\textbf{Colon}} &  \multirow{2}{*}{\textbf{Stomach}} &  \multirow{2}{*}{\textbf{Esophagus}} 
& \multirow{2}{*}{\textbf{Average}} \\
\cmidrule(rl){2-5} 
 & $S_{FC}$ & $S_{IC}$ & $S_{LRC}$ & $CoT_{e}$ & \\
 \midrule
Claude3-Haiku & 59.31 & 43.66 & 30.80 & 43.21 & 0000 & 0000 & 0000 & 0000 & 0000 & 0000 \\
Gemini2.0-Flash & 63.10 & 57.69 & 45.12 & 54.28 &  &  &  &  &  &  \\
GPT-5-Mini & 64.22 & 66.42 & 55.09 & 61.23 &  &  &  &  &  &  \\
\midrule
Qwen2.5-VL-7B & 49.15 & 22.89 & 12.09 & 26.45& \\
InternVL-2.5-8B & 56.66 & 57.92 & 47.05 & 53.19 & \\
MiniCPM-V-4.5-9B & 60.51 & 58.52 & 45.44 & 53.89 & \\
\midrule
HealthGPT-3.8B& 49.64 & 49.68 & 37.15 & 44.65 & \\
Lingshu-7B & 52.51 & 31.93 & 16.46 & 31.92&\\
MedVLM-R1-2B & 40.25 & 36.05 & 21.23 & 31.38 &  &  & &  &  \\
\midrule
\textbf{TumorChain-3B} & 62.37 & 49.99 & 35.68 & 47.98 &  &  &  &  &  &  \\
\textbf{TumorChain-7B} & 61.75 & 62.60 & 52.57 & 58.33 &  &  &  &  &  &  \\
\bottomrule
\end{tabular}
}
\end{center}
\end{table}
